Investigating Steady Unconfined Groundwater Flow using Physics Informed Neural Networks

A novel deep learning technique called Physics Informed Neural Networks (PINNs) is adapted to study steady groundwater flow in unconfined aquifers. This technique utilizes information from underlying physics represented in the form of partial differential equations (PDEs) alongside data obtained from physical observations. In this work, we consider the Dupuit-Boussinesq equation, which is based on the Dupuit-Forchheimer approximation, as well as a recent more complete model derived by Di Nucci (2018) as underlying models. We then train PINNs on data obtained from steady-state analytical solutions and laboratory based experiments. Using PINNs, we predict phreatic surface profiles given different input flow conditions and recover estimates for the hydraulic conductivity from the experimental observations. We show that PINNs can eliminate the inherent inability of the Dupuit-Boussinesq equation to predict flows with seepage faces. Moreover, the inclusion of physics information from the Di Nucci and Dupuit-Boussinesq models constrains the solution space and produces better predictions than solely the training data. PINNs based predictions are very robust and show little effect from added noise in the training data. Further, we compare the PINNs obtained using the two different flow models to examine the effects of higher order flow terms, which are neglected by the Dupuit Forchheimer approximation. We found a dimensionless parameter $\Pi$, which is the ratio of vertical to horizontal flow effects. For $\Pi \leq 0.1$, Dupuit-Boussinesq approximation is found to be applicable but not otherwise. Lastly, we discuss the effectiveness of using PINNs for examining groundwater flow.

==> trackchanges-0.7.0/README <==

TrackChanges
Multiple editors in LaTeX.
========================================================================

INTRODUCTION:

  The TrackChanges package consists of two parts:
  1.  A LaTex style file: 
        trackchanges.sty
  2.  A GUI, written in python:
         trackchanges.py

  The style file may be used without the GUI.  The GUI is to be used to
  facilitate accepting, rejecting, or modifying the edits made using the
  commands defined in the style file.

  This packages also includes a command line utility: acceptchanges.py.
  This utility will only work in posix environments.

  Help files are available as part of this package:
    ./documentation/web/help.html

  Documentation is also  available at the TrackChanges website.

  To get the latest version of this sofware go to:
    http://trackchanges.sourceforge.net

========================================================================

LaTeX STYLEFILE:

  INSTALLATION:
    Copy the style file to the directory with your LaTeX document.
    The style file can be found at: ./LatexPackage/trackchanges.sty

  USAGE:
    Add the following line to you latex document:
      \usepackage{trackchanges}

    Add the names of the editors in the preamble [OPTIONAL]:
      \addeditor{editor}

    Now you have access to all of the TrackChanges commands:
      \add[editor]{added text}
      \remove[editor]{removed text}
      \change[editor]{removed text}{added text}
      \note[editor]{note text}
      \annote[editor]{text to annotate}{note text}

    See the documentation or website for display options.

========================================================================

TRACKCHANGES GUI

  This is a Beta version of the TrackChanges GUI. 
  That means: Beware! Bugs may lurk ahead.

  If you choose to use this software plese be careful to back up your 
  TeX files.  This software has not been thoroughly tested and may
  corrupt your TeX files.  (The style file is fine and can't mess any
  thing up but the GUI for accepting/rejecting/modifying might.)

  ----------------------------------------------------------------------
  
  WARNING:  
    This program has not be generalized to handle international
    characters.  Such characters may cause unexpected behavior.
  
  NOTE:
    So far the GUI has only been tested on Windows XP and Os X.
    While it should work on linux, it might not.
  
  WARNING (AGAIN):
    This is beta software. It has not been tested much.
    Things may be broken.
  
  
  
  ----------------------------------------------------------------------
  INSTALLATION:
    Once you have all the dependencies installed, 
    just run ./PythonPackage/trackchanges.py
    
      $> cd PythonPackage
      $> python trackchanges.py
  
  
  ----------------------------------------------------------------------
  DEPENDANCIES:
    To get the trackchanges GUI to run you will need several things:
     
    1. Python 2.6 or later
    2. PyQt 4.4.4 or later
  
  ----------------------------------------------------------------------
  WHERE TO GET DEPENDANCIES:
    Python 2.6  -- http://www.python.org/
    PyQt 4      -- http://www.riverbankcomputing.co.uk/
  
  


========================================================================

This file is part of TrackChanges
Copyright 2009 Novimir Antoniuk Pablant
               Felix Salfner

TrackChanges is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 2 of the License, or
(at your option) any later version.

TrackChanges is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with TrackChanges.  If not, see <http://www.gnu.org/licenses/>.

------------------------------------------------------------------------
